MALADE: Orchestration of LLM-powered Agents with Retrieval Augmented Generation for Pharmacovigilance

In the era of Large Language Models (LLMs), given their remarkable text understanding and generation abilities, there is an unprecedented opportunity to develop new, LLM-based methods for trustworthy medical knowledge synthesis, extraction and summarization. This paper focuses on the problem of Pharmacovigilance (PhV), where the significance and challenges lie in identifying Adverse Drug Events (ADEs) from diverse text sources, such as medical literature, clinical notes, and drug labels. Unfortunately, this task is hindered by factors including variations in the terminologies of drugs and outcomes, and ADE descriptions often being buried in large amounts of narrative text. We present MALADE, the first effective collaborative multi-agent system powered by LLM with Retrieval Augmented Generation for ADE extraction from drug label data. This technique involves augmenting a query to an LLM with relevant information extracted from text resources, and instructing the LLM to compose a response consistent with the augmented data. MALADE is a general LLM-agnostic architecture, and its unique capabilities are: (1) leveraging a variety of external sources, such as medical literature, drug labels, and FDA tools (e.g., OpenFDA drug information API), (2) extracting drug-outcome association in a structured format along with the strength of the association, and (3) providing explanations for established associations. Instantiated with GPT-4 Turbo or GPT-4o, and FDA drug label data, MALADE demonstrates its efficacy with an Area Under ROC Curve of 0.90 against the OMOP Ground Truth table of ADEs. Our implementation leverages the Langroid multi-agent LLM framework and can be found at https://github.com/jihyechoi77/malade.

==> links.tex <==


see page 10 and 76+ (RxNorm details)
https://www.ohdsi.org/wp-content/uploads/2017/10/OHDSI-Vocabulary-CDM-Tutorial-2017-2017.10.11.pdf

RxNorm files
https://www.nlm.nih.gov/research/umls/rxnorm/docs/rxnormfiles.html
https://www.ohdsi.org/web/wiki/doku.php?id=documentation:vocabulary:drug
https://arpsp.cdc.gov/profile/antibiotic-use/all-classes




paper: https://arxiv.org/pdf/2402.01680.pdf
repo: https://github.com/taichengguo/LLM_MultiAgents_Survey_Papers

